Reducing Commutativity Verification to Reachability with Differencing Abstractions

Commutativity of data structure methods is of ongoing interest, with roots in the database community. In recent years commutativity has been shown to be a key ingredient to enabling multicore concurrency in contexts such as parallelizing compilers, transactional memory, speculative execution and, more broadly, software scalability. Despite this interest, it remains an open question as to how a data structure's commutativity specification can be verified automatically from its implementation. In this paper, we describe techniques to automatically prove the correctness of method commutativity conditions from data structure implementations. We introduce a new kind of abstraction that characterizes the ways in which the effects of two methods differ depending on the order in which the methods are applied, and abstracts away effects of methods that would be the same regardless of the order. We then describe a novel algorithm that reduces the problem to reachability, so that off-the-shelf program analysis tools can perform the reasoning necessary for proving commutativity. Finally, we describe a proof-of-concept implementation and experimental results, showing that our tool can verify commutativity of data structures such as a memory cell, counter, two-place Set, array-based stack, queue, and a rudimentary hash table. We conclude with a discussion of what makes a data structure's commutativity provable with today's tools and what needs to be done to prove more in the future.

==> cpa.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% ADT   & Method Names           & Property                  & Expected  & RV result  & RV time   & OEA result & OEA time   & OEB result & OEB time     %% bench
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Memory   & $\MM{read}{write}$     & $s1.x = y_1$          & \rTRUE    & \rTRUE     & { 1.239 } & \rTRUE     & { 1.260 } & \rUNKNOWN\rFAIL & \rTIMEOUT\ignore{ 1.324 }\\  %% m-read-write-phi1-s
Memory   & $\MM{read}{write}$     & $\textsf{true}$           & \rFALSE   & \rFALSE    & { 1.300 } &          - & - &           - & -\\  %% m-read-write-true-frv
Memory   & $\MM{write}{write}$    & $y_1 = x_1$       & \rTRUE    & \rTRUE     & { 1.231 } & \rTRUE     & { 1.228 } & \rUNKNOWN\rFAIL & \rTIMEOUT\ignore{ 1.248 }\\  %% m-write-write-phi1-s
Memory   & $\MM{write}{write}$    & $\textsf{true}$           & \rFALSE   & \rTRUE     & { 1.212 } & \rFALSE    & { 1.216 } &          - & -\\  %% m-write-write-true-foeA
Memory   & $\MM{read}{read}$      & $\textsf{true}$           & \rTRUE    & \rTRUE     & { 1.260 } & \rTRUE     & { 1.220 } & \rTRUE     & { 1.315 }\\  %% m-read-read-true-s
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Counter  & $\MM{decr}{isz}$       & $s1.x > 1$                & \rTRUE    & \rTRUE     & { 1.427 } & \rTRUE     & { 1.507 } & \rTRUE     & { 1.513 }\\  %% c-decr-isz-phi1-s
Counter  & $\MM{decr}{isz}$       & $\textsf{true}$           & \rFALSE   & \rFALSE    & { 1.410 } &          - & - &           - & -\\  %% c-decr-isz-true-frv
Counter  & $\MM{decr}{incr}$      & $s1.x > 1$                & \rTRUE    & \rTRUE     & { 1.432 } & \rTRUE     & { 1.474 } & \rTRUE     & { 1.504 }\\  %% c-decr-incr-phi1-s
Counter  & $\MM{decr}{incr}$      & $\textsf{true}$           & \rTRUE    & \rTRUE     & { 1.461 } & \rTRUE     & { 1.523 } & \rTRUE     & { 1.700 }\\  %% c-decr-incr-true-s
Counter  & $\MM{incr}{isz}$       & $s1.x > 1$                & \rTRUE    & \rTRUE     & { 1.454 } & \rTRUE     & { 1.497 } & \rTRUE     & { 1.563 }\\  %% c-incr-isz-phi1-s
Counter  & $\MM{incr}{isz}$       & $\textsf{true}$           & \rFALSE   & \rFALSE    & { 1.461 } &          - & - &           - & -\\  %% c-incr-isz-true-frv
Counter  & $\MM{incr}{incr}$      & $\textsf{true}$           & \rTRUE    & \rTRUE     & { 1.463 } & \rTRUE     & { 1.479 } & \rTRUE     & { 1.652 }\\  %% c-incr-incr-true-s
Counter  & $\MM{decr}{decr}$      & $\textsf{true}$           & \rFALSE   & \rTRUE     & { 1.487 } & \rTRUE     & { 1.487 } & \rTRUE     & { 1.686 }\\  %% c-decr-decr-true-frv
Counter  & $\MM{decr}{decr}$      & $s1.x > 1$                & \rTRUE    & \rTRUE     & { 1.533 } & \rTRUE     & { 1.475 } & \rTRUE     & { 1.496 }\\  %% c-decr-decr-phi1-s
Counter  & $\MM{isz}{isz}$        & $\textsf{true}$           & \rTRUE    & \rTRUE     & { 1.491 } & \rTRUE     & { 1.489 } & \rTRUE     & { 1.810 }\\  %% c-isz-isz-true-s


==> sources.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Implementation of SimpleSet-nf}

\begin{lstlisting}[style=MyC]
#include <assert.h>
#include <stdlib.h>

#define o_new(st) {                             \
    st = malloc(sizeof(struct state_t));        \
    st->a = -1; st->b = -1; }

#define o_add(st,rv,v) {                                                \
    if ((st)->a == -1 && (st)->b == -1) { (st)->a = v; rv = 1; } \
    else if ((st)->a != -1 && (st)->b == -1) { (st)->b = v; rv = 1; } \
    else if ((st)->a == -1 && (st)->b != -1) { (st)->a = v; rv = 1; } \
    else { rv = 0; } }

#define o_isin(st,rv,v) {                       \
    rv = 0;                                     \
    if ((st)->a == v) rv = 1;                   \
    if ((st)->b == v) rv = 1; }

#define o_clear(st,rv) { (st)->a = -1; (st)->b = -1; rv = 1; }

#define o_norm(st,rv) {                         \
    if ((st)->a > (st)->b) {                    \
      int t = (st)->b;                          \
      (st)->b = (st)->a;                        \
      (st)->a = t;                              \
    }                                           \
    rv = 0; }

\end{lstlisting}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Implementation of ArrayStack}

\begin{lstlisting}[style=MyC]
#define o_new(res) res = (struct state_t *)malloc(sizeof(struct state_t)); res->top = -1;

#define o_push(st,rv,v) { \
  if ((st)->top == (MAXSTACK-1)) {rv = 0;} \
  else { (st)->top++; (st)->a[(st)->top] = v; rv = 1; } }

#define o_pop(st,rv) {          \
  if ((st)->top == -1) rv = -1; \
  else rv = (st)->a[ (st)->top-- ]; }

#define o_isempty(st,rv) rv = ((st)->top==-1 ? 1 : 0)
\end{lstlisting}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Implementation of List}

\begin{lstlisting}[style=MyC]
#include <stdio.h>
#include <stdlib.h>

#define o_new(st) { st = malloc(sizeof(struct state_t)); st->end=-1; }

#define o_add(st,rv,v) {                        \
  rv = 1; \
  for (int i=0; i<=(st)->end; i++) {            \
    if ((st)->list[i] == v) { rv = 0; break; } \
  } \
  if (rv == 1 && (st)->end == LISTCAP) { rv = 0; } \
  else { (st)->list[(st)->end+1] = v;  (st)->end++; } }


#define o_rm(st,rv,v) {                         \
  rv = 0;                                       \
  for (int i =0; i<=(st)->end; i++) { \
      if ( (st)->list[i] == v) { \
        (st)->list[i] = (st)->list[(st)->end]; (st)->end--; rv = 1; break; \
      } } }

#define o_contains(st,rv,v) {                                                 \
    rv = 0;                                                             \
    for (int i =0; i<=(st)->end; i++) {                                 \
      if ( (st)->list[i] == v) {  rv = 1; break; } \
    } }

#define o_isempty(st,rv) rv = ((st)->end > -1 ? 1 : 0)
\end{lstlisting}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Implementation of Counter}

\begin{lstlisting}[style=MyC]
#include <stdlib.h>

#define o_new(res) res = (struct state_t *)malloc(sizeof(struct state_t))
#define o_close(src) {                          \
    struct state_t* tmp;                        \
    o_new(tmp);                                 \
    tmp->x = src->x;                            \
    dst = tmp;                                  \
  }
#define o_incr(st,rv) { (st)->x += 1; rv = 0; }
#define o_clear(st,rv) { (st)->x = 0; rv = 0; }
#define o_decr(st,rv) { if ((st)->x == 0) rv = -1; else { (st)->x -= 1; rv = 0; } }
#define o_isz(st,rv) { rv = ((st)->x == 0 ? 1 : 0); }
\end{lstlisting}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Implementation of Accum.}

\begin{lstlisting}[style=MyC]
#include <stdlib.h>

#define o_new(res) res = (struct state_t *)malloc(sizeof(struct state_t))
#define o_close(src) {                          \
    struct state_t* tmp;                        \
    o_new(tmp);                                 \
    tmp->x = src->x;                            \
    dst = tmp;                                  \
  }
#define o_incr(st,rv) { (st)->x += 1; rv = 0; }
#define o_decr(st,rv) { (st)->x -= 1; rv = 0; }
#define o_isz(st,rv) { rv = ((st)->x == 0 ? 1 : 0); }
\end{lstlisting}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Implementation of Queue}

\begin{lstlisting}[style=MyC]
#include <stdlib.h>

#define o_new(res) { \
  res = malloc(sizeof(struct state_t)); \
  res->front = 0; \
  res->rear = MAXQUEUE-1; \
  res->size = 0; \
}

#define o_enq(st,rv,v) { \
  if((st)->size == MAXQUEUE) rv = 0; \
  else { \
    (st)->size++; (st)->rear = ((st)->rear + 1) % MAXQUEUE; (st)->a[(st)->rear] = v; rv = 1; } }

#define o_deq(st,rv) { \
  if((st)->size==0) rv = -1; \
  else { int r = (st)->a[(st)->front]; \
         (st)->front = ((st)->front + 1) % MAXQUEUE; \
         (st)->size--; \
         rv = r; } }

#define o_isempty(st,rv) rv = ( (st)->size==0 ? 1 : 0)
\end{lstlisting}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Implementation of Memory}

\begin{lstlisting}[style=MyC]
#include <stdlib.h>

#define o_new(res) res = (struct state_t *)malloc(sizeof(struct state_t))

#define o_clone(src) { \
  struct state_t* tmp; \
  o_new(tmp); \
  tmp->x = (src)->x;                            \
  dst = tmp; \
  }

#define o_read(st,rv)    rv = (st)->x
#define o_write(st,rv,v) { (st)->x = v; rv = 0; }


\end{lstlisting}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Implementation of SimpleSet}

\begin{lstlisting}[style=MyC]
#include <assert.h>
#include <stdlib.h>

#define o_new(st) {  \
  st = malloc(sizeof(struct state_t)); \
  st->a = -1; st->b = -1; st->filled = 0; }

#define o_add(st,rv,v) { \
  (st)->filled = (st)->filled+0; \
  if ((st)->a == -1 && (st)->b == -1) { (st)->a = v; (st)->b=(st)->b+0; rv = 0; } \
  else if ((st)->a != -1 && (st)->b == -1) { (st)->b = v; (st)->a=(st)->a+0; (st)->filled++; rv = 0; } \
  else if ((st)->a == -1 && (st)->b != -1) { (st)->a = v; (st)->b=(st)->b+0; (st)->filled++; rv = 0; } \
  else { rv = 0; } }

#define o_isin(st,rv,v) { \
  (st)->filled = (st)->filled+0; \
  rv = 0; \
  if ((st)->a == v) rv = 1; \
  if ((st)->b == v) rv = 1; }

#define o_wasFilled(st,rv) { rv = ((st)->filled > 0 ? 1 : 0); }

#define o_clear(st,rv) { (st)->a = -1; (st)->b = -1; (st)->filled = (st)->filled+0; rv = 0; }

#define o_norm(st,rv) { \
  if ((st)->a > (st)->b) { \
    int t = (st)->b; \
    (st)->b = (st)->a; \
    (st)->a = t; \
  } \
  rv = 0; }
\end{lstlisting}




==> stamp.tex <==
\subsection{Case study: Commutativity of STAMP Benchmarks}

\texttt{kmeans}.
transactions in a nested loop.\\
we collect this transaction as an operation.\\
increment (read/modify/write)\\
proved that \TRUE\ is a valid commutativity condition.


==> xform.tex <==
\begin{figure}[t]
  For an input object CFA $\aut_o$ and method signatures $m(\Xs),n(\Ys)$,
  the transformation yields output automaton
  $
  \autencMmn{\varphi_m^n} = (Q_\enc,X_\enc,s_\enc,\earrow{\ })
  $
  where
\[\begin{array}{ll}
Q_\enc &= \{ q_0, q_{er}, \\
X_\enc &= X_o \cup \{ o_1, o_2, r_m, r_n, r_{mn}, r_{nm}, r_1, r_2 \}\\
s_\enc &::= s \mid *_\textrm{Int} \mid ...
\end{array}\]

$$q_0 \earrow{\ \texttt{call } \texttt{SimpleSet()} }
\cdots
\earrow{\ \texttt{return} } q_0'
\earrow{o_1 := \textsf{this}_o } q_1
$$

$$
\forall m\in M.\ q_1 \earrow{ \As := \bar{*}_\textrm{Int} }
q_1^m \earrow{ \texttt{call } m(\As) } \cdots \earrow{\texttt{return}}  q_1
$$

$$
q_1 \earrow{ \texttt{assume}(\varphi_m^n) } q_1'
\earrow{\ \red{clone} }
\cdots
\earrow{\ \texttt{return} } q_1''
\earrow{o_2 := \textsf{this}_o } q_1'''
\earrow{\As := \bar{x}_\textrm{Int} } q_1'''
\earrow{\Bs := \bar{x}_\textrm{Int} } 
q_2
$$

$$
q_2 \earrow{ r_m := \texttt{call } m(\red{o_1},\As) }
\cdots \earrow{ r_{mn} := \texttt{call } n(\red{o_1},\Bs) }
q_2 \earrow{ r_n := \texttt{call } n(\red{o_2},\Bs) }
\cdots \earrow{ r_{nm} := \texttt{call } m(\red{o_2},\Bs) }
\red{abbrev?}
$$
\caption{\label{fig:trans} Transformation from input
  object automaton $\aut_o$ to encoding $\autencMmn{\varphi_m^n}$. Non-reachability of $q_{er}$ in $\autencMmn{\varphi_m^n}$ entails
  that $\varphi_m^n$ is a commutativity condition. Existence of
  a terminating run entails that $\varphi_m^n$ is a \emph{non}-commutativity
  condition.}
\end{figure}

